LISA: Learning Implicit Shape and Appearance of Hands

This paper proposes a do-it-all neural model of human hands, named LISA. The model can capture accurate hand shape and appearance, generalize to arbitrary hand subjects, provide dense surface correspondences, be reconstructed from images in the wild and easily animated. We train LISA by minimizing the shape and appearance losses on a large set of multi-view RGB image sequences annotated with coarse 3D poses of the hand skeleton. For a 3D point in the hand local coordinate, our model predicts the color and the signed distance with respect to each hand bone independently, and then combines the per-bone predictions using predicted skinning weights. The shape, color and pose representations are disentangled by design, allowing to estimate or animate only selected parameters. We experimentally demonstrate that LISA can accurately reconstruct a dynamic hand from monocular or multi-view sequences, achieving a noticeably higher quality of reconstructed hand shapes compared to baseline approaches. Project page: https://www.iri.upc.edu/people/ecorona/lisa/.

==> figure_teaser_v2.tex <==
\begin{figure}[t!]
\noindent\includegraphics[width=0.95\linewidth]{images/teaser_v2.png}\\
\label{fig:freihand}
  \caption{\small{{\bf Caption}, First row: reconstruction, second row: changing pose, third row: changing shape, fourth row: changing color. We need the reconstructed geometry and skinning weights in the colours we've used in the remaining figures, and then update the figure, labels, sizes, etc.}}
\end{figure}

==> section_implementation_details.tex <==

\section{Implementation details}\label{sec:implem}

==> table_noise_in_joints.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.9 \textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c c c c c}
\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
& & \multicolumn{4}{c}{1 view} & \multicolumn{4}{c}{2 views} & \multicolumn{4}{c}{4 views} \\

Noise & GT Joint error & PSNR  & V2V & V2S & Joint error & PSNR  & V2V & V2S & Joint error & PSNR  & V2V & V2S & Joint error \\

\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}

$\sigma=0$ & & 25.43 & 3.84 & 3.68 & 8.63  & 29.40 & 3.70 & 3.56 & 6.81 & 29.69 & 3.53 & 3.38 & 6.17 \\
$\sigma=2mm$ & & 25.18 & 3.99 & 3.84 & 8.65  & 29.27 & 3.71 & 3.56 & 7.01 & 29.50 & 3.71 & 3.55 & 6.21 \\
$\sigma=5mm$ & & 24.86 & 4.18 & 4.04 & 8.43  & 28.93 & 4.06 & 3.92 & 7.40 & 28.91 & 3.99 & 3.86 & 6.65 \\
$\sigma=10mm$ & & 24.20 & 5.50 & 5.39 & 12.19  & 28.41 & 4.84 & 4.71 & 8.62 & 28.38 & 4.44 & 4.32 & 7.16 \\
$\sigma=20mm$ & & 24.19 & 6.96 & 6.87 & 17.32  & 27.99 & 5.75 & 5.63 & 10.46 & 27.59 & 5.01 & 4.90 & 8.76 \\

\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
\end{tabular}}
\caption{\small{{\bf DeepHandMesh.}. How 3D reconstructions are affected by noise in input 3D joints. \enric{This for supplementary.}}}
\label{tab:sensitiveness_joint_noise}
\end{table*}


